Requirements Elicitation in Government Projects: A Preliminary Empirical Study

Government development projects vary significantly from private sector initiatives in scope, stakeholder complexity, and regulatory requirements. There is a lack of empirical studies focusing on requirements engineering (RE) activities specifically for government projects. We addressed this gap by conducting a series of semi-structured interviews with 12 professional software practitioners working on government projects. These interviewees are employed by two types of companies, each serving different government departments. Our findings uncover differences in the requirements elicitation phase between government projects, particularly for data visualization aspects, and other software projects, such as stakeholders and policy requirements. Additionally, we explore the coverage of human and social aspects in requirements elicitation, finding that culture, team dynamics, and policy implications are critical considerations. Our findings also pinpoint the main challenges encountered during the requirements elicitation phase for government projects. Our findings highlight future research work that is important to bridge the gap in RE activities for government software projects.

==> Section/todo.tex <==
%%%%%----From a methodological perspective, the research seems sound. However, some aspects are not adequately described, which I indicate below. None of these aspects represents a significant threat to validity, except for the knowledge and experience of participants in RE tasks, data visualization, and other projects, which would affect the credibility of the information provided in the interviews.


%%%%One aspect contributing to the doubts above is that non-governmental systems need to be better described. For the findings to be genuinely representative, a study of such systems (preferably, data visualization projects carried out in industry) and an explicit comparison with governmental systems would be necessary. ---- in limitations


%%%%%As mentioned above, we need to understand the differences between government projects and other types of software projects" --> Visualization projects in big companies, e.g., Amazon or Microsoft, may share many of the characteristics of government projects. Is it the domain that really matters or the project context?

Our findings revealed that government data visualization projects differ from other software projects." Please clarify how the interviews provide information to reach this conclusion.

Related work:

- The first part of the Related Work Section, which is related to data visualization within the software engineering life cycle, does not seem to be connected to the research goal.

- Similarly, Matheus et al. [30] do not address visualization for government but for RE.

- Reference [32] suffers the same problem. Unless I misinterpret the research, I cannot see why works related to requirements visualization are relevant to government data visualization.

Related method:

- Please provide more context about government projects, e.g., which administration promotes them, what the project goals are, etc.

- To what extent are the participants involved in requirements tasks? Do they have experience in projects different than data visualization (which is relevant to assess whether they have enough knowledge to indicate differences between data visualization and other projects)?

“We specifically asked interviewees to discuss the influence of cultural aspects" --> Which aspects in particular? Hidellaarachchi et al. [2], [18] describe the human and social aspects, but the paper does not mention the cultural aspects.



review2:

The design of the study lacks a meaningful comparison against projects without government visualisation. All the interviewed participants worked at companies doing government visualisation projects, and we do not know about their prior experience. I was expecting a second set of interview participants who worked at non-government visualisation projects, and then I was expecting the authors to perform some kind of qualitative comparison analysis across the two sets of interview notes. This is not the case. The entire results rely on the presumed dual knowledge of the participants, which is a major threat to validity.


- There are no methodological details about the Thematic Analysis, and their only research reference is to Thematic Synthesis, which is a different method. They have neither described any of their pre-decisions of the analysis (inductive vs deductive, semantic vs latent themes, etc.), nor any of the complexities of the different five phases of standard thematic analysis. Additionally, they have not provided a replication package showing the evidence for their claims. Thematic Analysis is a rigorous method where evidence tracing should be applied (even in the case of full anonymisation, we should see the surrounding evidence tracing framework).


- The article is missing a replication package that includes their scientific artefacts, such as their interview guidelines. This is important because they mentioned that these guidelines evolved *during the interviews*. Therefore, it is reasonable to assume that reviewers and readers alike would want to see all versions of these guidelines, and make a judgement call on the validity of the procedure, given these evolutions.


Grammar issue: "Requirements Engineering (RE) is an important social technical activities involving various types of stakeholders ..."
- Missing Reference: "Among these, the effectiveness of requirements elicitation directly impacts whether the system is successful."
- "Hence, we use government data visualisation projects and government projects interchangeably." → I don't think this is a suitable substitution to make. In this article the authors use "visualisation" about half of the times they mention "government projects", which may confuse readers as to what the other half of the occurrences mean.
- I am missing a definition of what "government visualisation projects" are. Somewhere in the first paragraph, the authors should describe what they mean by this. There are many possible definitions for this, but the reader should know what the authors really mean by this expression right from the beginning.
- "Safeguarding this sensitive data against unauthorized access or disclosure represents a significant challenge during the data visualisation process [11]." The authors appear to be using this reference in the wrong place. None of the primary keywords the authors used are mentioned in this reference: safeguarding, sensitive data, unauthorised access, disclosure, etc. Additionally, the incorrect reference is used. It should be: "Esteban Ortiz-Ospina and Max Roser (2016) - “Government Spending” Published online at OurWorldInData.org. Retrieved from: 'https://ourworldindata.org/government-spending' [Online Resource]". The article ever provides the proper BibTeX at the bottom.
- "Government data visualisation projects play a critical role in the social, political and technological environments [11]." Similar issue with primary keywords not being present. This referenced article is about government spending, not government visualisation projects.
- "However, there is a lack of empirical research on the RE for government projects that we aim to address in this paper and in future." → It is not clear to me what the authors mean by "government projects" here. Are they referring to internal projects, projects that reach citizens, or perhaps something different? The authors do not provide any meaningful context.

Section 3: Research Method
- "To ensure the quality of the interview data, we also iteratively refined our interview guidelines after the second and seventh interviews." → This may have improved the quality of the subsequent interviews, but it may also have introduced some threats to validity when comparing and combining results across interviews. It doesn't appear that the authors have shared a replication package with these different evolutions of the interview guidelines, thereby further introducing uncertainty as to the validity of their work.
- "We also asked interviewees to provide recent examples of government data visualisation projects and discussed the differences in eliciting user requirements between government data visualisation projects and other types of visualisation projects, such as business or customer projects." → Have these participants worked in positions apart from government visualisation projects? How can they give meaningful comments on this otherwise?
- "Then, we conducted a thematic analysis to code the entire transcripts using MAXQDA, following recommended practices [35]–[37]." → You have not presented any details of your thematic analysis. Is it inductive or deductive? Are you applying semantic or latent themes? Which epistemological lens are you applying: Essentialist/Realist or Constructionist? What happened in the different phases of your analysis? Where is the replication package showing your qualitative work to arrive at your findings?

Section 4: Findings
- I'm not convinced that the findings regarding "Stakeholders" really are all that different from traditional RE projects: there are always unique stakeholder groups. This should be considered and discussed in more detail than just taking what the interviewees say at face value. This is a comparison to the "Policy Requirements" results, which do seem well differentiated and described.
